The Decision Problem for Regular First-Order Theories

The \emph{Entscheidungsproblem}, or the classical decision problem, asks whether a given formula of first-order logic is satisfiable. In this work, we consider an extension of this problem to regular first-order \emph{theories}, i.e., (infinite) regular sets of formulae. Building on the elegant classification of syntactic classes as decidable or undecidable for the classical decision problem, we show that some classes (specifically, the EPR and Gurevich classes), which are decidable in the classical setting, become undecidable for regular theories. On the other hand, for each of these classes, we identify a subclass that remains decidable in our setting, leaving a complete classification as a challenge for future work. Finally, we observe that our problem generalises prior work on automata-theoretic verification of uninterpreted programs and propose a semantic class of existential formulae for which the problem is decidable.

==> qfree-congruence.tex <==
%!TEX root=./main.tex

\subsection{Congruence closure}

\begin{definition}
Let $E=\{s_i=t_i\}$ be a set of equality constraints.  Define the relation $R$ to be the smallest equivalence relation on $\Ss^*$ \um{What is $\Ss^*$} such that
\begin{itemize}
    \item $(s_i,t_i) \in R$ for all $s_i=t_i\in E$, and
    \item $R$ is a \emph{congruence}: for any function symbol $f$ of arity $k$ and terms $a_1,\ldots,a_k,b_1,\ldots,b_k$ with $(a_i,b_i)\in R$ for all $i$, we have $(f(a_1,\ldots,a_k),f(b_1,\ldots,b_k))\in R$.
\end{itemize}
Let $S\subseteq \Ss^*$ be any set of terms.  Define the \emph{congruence closure of $S$ under $E$}, $\congclos_E(S)$, to be the set of terms related by $R$ to elements of $S$.
\end{definition}

The reason why congruence closure is useful for EUF is that it is sufficient to tell us whether a set of EUF constraints is satisfiable. 

\begin{proposition}\label{prop:congsound}
Let $T=E\cup D$, where $E$ and $D$ are sets of equality and disequality atomic propositions respectively.  Then $\bigwedge T$ is unsatisfiable if and only if there exists a disequality $t\neq t' \in D$ such that $t' \in \congclos_E(\{t\})$.
\end{proposition}

The main theorem of this subsection is that if $S$ is a regular set of terms then the congruence closure of $S$ under equating the elements of regular sets $S_1,\ldots,S_n$ is itself regular, and is computable as a function of the inputs.

\dm{https://www.sciencedirect.com/science/article/pii/089054019090015A remark at the bottom of p.195}

\begin{theorem}\label{thm:congclos}
Let $\Aa,\Aa_1,\ldots,\Aa_n$ be tree automata.  Let $E=\{s=t|s,t\in L(\Aa_i) \text{ for some $i$}\}$.  Then $\congclos_E(L(\Aa))$ is regular, and given by an automaton computable as a function of $\Aa,\Aa_1,\ldots,\Aa_n$.
\end{theorem}

Fix $S=L(\Aa)$ and $S_i=L(\Aa_i)$.  The algorithm to compute $\congclos_E(S)$ proceeds as follows:
\begin{itemize}
    \item Form the automaton $\Aa'=\Aa \sqcup \Aa_1 \sqcup \ldots \sqcup \Aa_n$, with accepting state the accepting state of $\Aa$.  Let the accepting states of the $\Aa_i$ be denoted by $q_i$.
    \item Repeatedly apply the $\grow$ operation to $\Aa'$ until stability, where grow consists of testing for every state $q$ and every $i$ whether $L(q)\cap S_i$ is non-empty, and if so adding a silent transition $q_i \rightarrow q$ (if not already present).
\end{itemize}

This clearly terminates, since $\grow$ adds new transitions but not new states, so it remains to prove that $L(\grow^\omega(\Aa')) = \congclos_E(S)$.  In order to prove that this operation on automata corresponds to the set of terms for which there exist proofs of congruence using the transitivity and congruence rules, we will define two distinct but related functions on sets of terms, show that both have congruence closure as their least fixed point, and finally use their relationship to $\grow$ to show that $\grow^\omega$ also gives the congruence closure.

The first function, $\subst$, is given by substituting subterms of the input term which are in some $S_i$ with another element of $S_i$, possibly for several subterms at the same time (and several $i$); more formally, for any set of terms $L$ define 
\begin{align*}
\subst&(L) = \{t\in \Ss^*|\exists s\in L \text{ s.t. $\exists$ context $C$ and terms } t_1,t'_1,\ldots,
t_k,t'_k \text{ s.t. for all $i$, }\\
&t_i,t'_i\in S_j \text{ for some $j$, and } s=C[t_1/X_1,\ldots,t_k/X_k] \text{ and } t=C[t'_1/X_1,\ldots,t'_k/X_k]\}.
\end{align*}

\begin{lemma}\label{lem:substom}
For any set $L$, $\subst^\omega(L)=\congclos_E(L)$, where $E=\{s=t|s,t \in S_i \text{ for some $i$}\}$.
\end{lemma}
\begin{proof}
Clearly $\subst^\omega(L) \subseteq \congclos_E(L)$: indeed, $\subst(L) \subseteq \congclos_E(L)$ (since $t_i=t'_i \in E$ for all $i$ and hence $(s,t)\in R$ by congruence), so also $\subst^\omega(L) \subseteq \congclos_E(L)$.

For the converse, note that it suffices to consider singleton sets $L=\{t\}$.  We will proceed by induction on the length of the congruence proof, but some care is required: we have to perform the induction simultaneously for all singletons $t$.  Thus our inductive hypothesis is `for all $t$, $\kcc{k}_E(\{t\}) \subseteq \subst^\omega(\{t\})$', where $\kcc{k}(L)$ is the set of elements with congruence closure proofs from $L$ of length at most $k$.  The base case is trivial since $\kcc{0}(L)=L$.

Now suppose that $t'\in \kcc{(k+1)}(\{t\})$.  The final step of the congruence proof is either
\[\text{(trans): }t=s, s=t \Rightarrow t=t'\]
or
\[\text{(cong): }s_1=s'_1,\ldots,s_m=s'_m \Rightarrow t=f(s_1,\ldots,s_m)=f(s'_1,\ldots,s'_m)=t',\]
and we consider the two cases separately.

Case (trans): since $t=s$ and $s=t'$ appeared as conclusions in the first $k$ steps of the proof, we have $s\in \kcc{k}(\{t\})$ and $t'\in \kcc{k}(\{s\})$.  Hence by the inductive hypothesis $s\in \subst^\omega(\{t\})$, so $\subst^\omega(\{s\})\subseteq \subst^\omega(\{t\})$.  Also by the inductive hypothesis we have $t'\in \subst^\omega(\{s\})$ and so $t'\in \subst^\omega(\{t\})$, as required.

Cast (cong): by the inductive hypothesis we have $s'_i\in \subst^\omega(\{s_i\})$, and hence $t'\in f(\subst^\omega(\{s_1\}),\ldots,\subst^\omega(\{s_m\})) \subseteq \subst^\omega(\{f(s_1,\ldots,s_m)\}) = \subst^\omega(\{t\})$, as required.
%(note that it is immediate from the definition of $\subst$ that for any $L_1,\ldots,L_m$ we have $f(\subst(L_1),\ldots,\subst(L_m)) \subseteq \subst(f(L_1,\ldots,L_m))$).
\end{proof}

Now it is easy to see that $\subst(L(\grow^k(\Aa'))) \subseteq L(\grow^{k+1}(\Aa'))$.  Indeed, if $t\in \subst(L(\grow^k(\Aa')))$ then $\exists s\in L(\grow^k(\Aa'))$ and context $C$ and terms $t_1,t'_1,\ldots,t_k,t'_k$ with each $t_i,t'_i \in S_{j_i}$ for some $j_i$ and $s=C[t_1/X_1,\ldots,t_m/X_m]$, $t=C[t'_1/X_1,\ldots,t'_m/X_m]$.  Since $s\in \grow^k(\Aa')$ there must exist states $q'_1,\ldots,q'_m$ such that in $\grow^k(\Aa')$ we have $t_i\in L(q'_i)$ and $q'_1(X_1),\ldots,q'_m(X_m)\rightarrow \qacc(C)$.  Since $t_i \in L(q'_i)\cap S_{j_i}$ we have that in $\grow^{k+1}(\Aa')$ there is a silent transition $q_{j_i} \rightarrow q'_i$ and so $S_{j_i}\subseteq L(q'_i)$ and in particular $t'_i\in L(q'_i)$, and hence $t\in L(\grow^{k+1}(\Aa'))$, as required.  Combining this with Lemma \ref{lem:substom} gives
\begin{equation}\label{eq:substom}\subst^\omega(L(\Aa')) = \congclos_E(L(\Aa')) \subseteq L(\grow^\omega(\Aa')).\end{equation}

For the reverse containment, we define a slightly stronger function $\subst'$, which allows substituting subterms in $S_i$ not only by other elements of $S_i$ but of $\subst^\omega(S_i)$; formally, for any set $L$ define

\begin{align*}
\subst'&(L) = \{t\in \Ss^*|\exists s\in L \text{ s.t. $\exists$ context $C$ and terms } t_1,t'_1,\ldots,
t_k,t'_k \text{ s.t. for all $i$, }\\
&t_i\in S_j, t'_i \in \subst^\omega(S_j) \text{ for some $j$, and } s=C[t_1/X_1,\ldots,t_k/X_k] \text{ and }\\
&t=C[t'_1/X_1,\ldots,t'_k/X_k]\}.
\end{align*}

Unsurprisingly, a single application of $\subst'$ can be obtained as a repeated application of $\subst$ and so it has the same least fixed point as $\subst$:

\begin{lemma}\label{lem:substpom}
For any set $L$, $\subst'^\omega(L)=\subst^\omega(L)$.
\end{lemma}
\begin{proof}
Trivially $\subst'^\omega(L) \supseteq \subst^\omega(L)$.  For the converse, it suffices to prove $\subst'(L) \subseteq \subst^\omega(L)$.  We will prove by induction on $k$ that $\subst'_k(L) \subseteq \subst^\omega(L)$, where $\subst'_k$ is defined as $\subst'$ where each of the $t'_i\in \subst^k(S_j)$.  The base case is trivial since $\subst'_0=\subst$.

Now say $t\in \subst'_{k+1}(L)$, so $t=C[t'_1/X_1,\ldots,t'_m/X_m]$ for some $t'_i\in \subst^{k+1}(S_{j_i})$, and $C[t_1/X_1,\ldots,t_m/X_m] \in L$ for some $t_i \in S_{j_i}$.  Since each $t'_i\in \subst^{k+1}(S_{j_i})$, we have $t'_i=C_i[t'_{i,1}/X_{i,1},\ldots,t'_{i,m_i}/X_{i,m_i}]$ and $C_i[t_{i,1}/X_{i,1},\ldots,t_{i,m_i}/X_{i,m_i}]\in \subst^k(S_{j_i})$ for some context $C_i$ and terms $t_{i,j}, t'_{i,j}\in S_{k_{i,j}}$ for some $S_{k_{i,j}}$.  But then we have
\[t = (C[C_1/X_1,\ldots,C_m/X_m])[t'_{1,1}/X_{1,1},\ldots,t'_{2,1}/X_{2,1},\ldots],\]
and 
\begin{align*}
    t' := (C[C_1/&X_1,\ldots,C_m/X_m])[t_{1,1}/X_{1,1},\ldots,t_{2,1}/X_{2,1},\ldots,t_{m,1}/X_{m,1},\ldots] \\ 
    &= C[C_1[t_{1,1}/X_{1,1},\ldots]/X_1,\ldots,C_m[t_{m,1}/X_{m,1},\ldots]/X_m] \\
    &\in \subst'_k(L)
\end{align*}
since each of the $C_i[t_{i,1}/X_{i_1},\ldots]\in \subst^k(S_{j_i})$ and $C[t_1/x_1,\ldots]\in L$.  By the inductive hypothesis $\subst'_k(L)\subseteq \subst^\omega(L)$ and so $t'\in \subst^\omega(L)$ and $t\in \subst(\{t'\}) \subseteq \subst^\omega(L)$, as required.
\end{proof}

We are now ready to complete the proof of Theorem \ref{thm:congclos}.  We will prove by induction on $l$ that for any state $q$ we have $L_{\grow^l(\Aa')}(q) \subseteq \subst^\omega(L_\Aa'(q))$.  To do this, for fixed $l$ we show by induction on $k$ that for every term $t$ with an accepting run of size at most $k$, if $t\in L_{\grow^{l}(\Aa')}(q)$ then $t\in \subst^\omega(L_{\Aa'}(q))$.

Let $t$ be such a term.  Unless $t\in L_{\grow^{l-1}}(\Aa')(q)$, we have $t=C[t'_1/X_1,\ldots,t'_m/X_m]$, where $t'_i\in L_{\grow^l(\Aa')}(q_{j_i})$ for some $j_i$, $q_{j_i}\rightarrow q'_i$ are new silent transitions inserted by the $l$th application of $\grow$ and in $\grow^{l-1}(\Aa')$ we have $q'_1(X_1),\ldots,q'_m(X_m)\rightarrow q(C)$ and this forms part of a minimum-size run for $q(t)$ in $\grow^l(\Aa')$ (intuitively, we are cutting up a minimum accepting run for $t$ at the first places newly-added transitions are taken). 

Now since the $q_{j_i}\rightarrow q'_i$ transitions were inserted, we must have $t_i\in L_{\grow^{l-1}(\Aa')}(q'_i)$ for some $t_i\in S_{j_i}$.  Since $q'_1(X_1),\ldots,q'_m(X_m) \rightarrow q(C)$ in $\grow^{l-1}(\Aa')$, we have that $C[t_1/X_1,\ldots,t_m/X] \in L_{\grow^{l-1}(\Aa')}(q) \subseteq \subst^\omega(L_{\Aa'}(q))$ by the inductive hypothesis on $l$. Also the $t'_i$ must have accepting runs in $L_{\grow^l(\Aa')}(q_{j_i})$ of size less than $k$, and so by the inductive hypothesis on $k$ we have $t'_i\in \subst^\omega(L_{\Aa'}(q_{j_i})) = \subst^\omega(S_{j_i})$.  Hence we have that $t\in \subst'(\subst^\omega(L_{\Aa'}(q))) = \subst^\omega(L_{\Aa'}(q))$ by Lemma \ref{lem:substpom}, as required.

Taking $q=\qacc$ gives $L(\grow^\omega(\Aa')) \subseteq \subst^\omega(L(\Aa'))$.  Combining this with equation (\ref{eq:substom}) completes the proof of Theorem \ref{thm:congclos}. \qed

==> qfree-disjunctive.tex <==
%!TEX root=./main.tex

\subsection{Decidability of disjunction \um{DEAD, more or less}.}


\um{Commented out in the source.}


\begin{comment}
\begin{theorem}\label{thm:quantfreedis}
The problem of determining whether $\bigvee T$ is satisfiable, where $T=L(\Aa)$ is a given regular purely existential theory, is decidable.
\end{theorem}

We will prove this by reduction to essentially the same special case as for the proof of Theorem \ref{thm:quantfreecon}.  The reduction itself is the same as before, but as we will see the proof of decidability is rather more involved.  The key idea is that infinite sets of possible equalities can always be satisfied since they can be instantiated with terms far bigger than any used to satisfy disequality constraints; the complication is that finite equality constraints can make everything a little more subtle.

\begin{lemma}\label{lem:ignoreinf}
\um{This is now a conjecture.}
Let $E$ be a finite set of equality atomic propositions and $S_1,S'_1,\ldots,S_n,S'_n$, $T_1,T'_1,\ldots,T_m,T'_m$ regular sets of terms such that 
\begin{enumerate}[label=(\roman*)]
\item For all $j$, $\exists t\in T_j, t'\in T'_j$ with $t'\not\in \congclos_E(\{t\})$, and
\item For all $i$, $S_i$ contains infinitely many non-equivalent terms under $E$.
\end{enumerate}
Then $\bigvee T$ is satisfiable, where 
\[T = \left\{\bigwedge E \wedge s_1=s'_1 \wedge \ldots \wedge s_n=s'_n \wedge t_1 \neq t'_1 \wedge \ldots \wedge t_m \neq t'_m \mid s_i \in S_i, s'_i \in S'_i, t_j\in T_j, t'_j\in T'_j\right\}.\]
\end{lemma}

%\dm{Idea: suppose $s=s_{massive}$ causes $t_i =t_j$.  When is the last time $s_{massive}$ is substituted ina production of minimum length?  This yields a term in the class of $t_j$ which has $s_{massive}$ as a subterm, contradiction.}

To show this, first for each $j$ fix $t_j \in T_j, t'_j \in T'_j$ with $t'_j\not\in \congclos_E(\{t_j\})$, and for each $i$ fix arbitrary $s'_i\in S'_i$.  We will choose an $s_i\in S_i$ for each $i$ such that no element of $\congclos_E(t_j), \congclos_E(t'_j)$ or $\congclos_E(s'_{i'})$ for any $i',j$, or $\congclos_E(s_{i'})$ for any $i'\neq i$, or $\congclos_E(s)$ or $\congclos_E(t)$ for any $s=t\in E$, contains as a subterm an element of $\congclos_E(s_i)$, and such that $\congclos_E(s_i)$ does not contain a strict subterm of $s_i$; we will show that this is possible by Lemma XXX below.

Having chosen the $s_i$ in this way, we claim that \[\phi = \bigwedge E \wedge s_1=s'_1 \wedge \ldots \wedge s_n=s'_n \wedge t_1 \neq t'_1 \wedge \ldots \wedge t_m \neq t'_m \in T\] is satisfiable.  Indeed, let $E'=\{s_i=s'_i\}_{i=1}^n$; then it suffices to prove that $t'_j \not\in \congclos_{E\cup E'}(\{t_j\})$ for all $j$.  We will say that a term $s$ `appears in' $E$ if $s=t\in E$ or $t=s\in E$ for some $t$.

Suppose to the contrary $t'_j \in \congclos_{E\cup E'}(\{t_j\})$.  Then by Lemma \ref{lem:substom} it is possible to reach $t'_j$ from $t_j$ by a sequence of substitutions from $E\cup E'$, so consider a minimum length sequence.  If any substitutions of the form $s_i/s'_i$ occur, consider the last such substitution---say this produces a term $t$ with $s_i$ as a subterm.  Inside this subterm no further $E'$ substitutions can occur: $s_{i'}/s'_{i'}$ substitutions are prevented because we assumed this was the last such substitution, and $s'_{i'}/s_{i'}$ substitutions are prevented because no $s_{i'}$ is a subterm of a term equivalent to $s_i$ under $E$ (consider the first such substitution; all previous substitutions must have been by elements of $E$).  Hence also no substitutions (weakly) containing the subterm can occur except for $s'_{i}/s_{i}$, since no term equivalent to $s_i$ under $E$ is a subterm of any $s_{i'}$ for $i'\neq i$ or of any $s$ appearing in $E$.  If the substitution $s'_{i}/s_{i}$ occurs it must be precisely of the subterm itself (since $s_i$ is not equivalent under $E$ to any strict subterm of itself), contradicting minimality (since we could just omit both substitutions).  Hence no further $E'$ substitutions occur, so a term equivalent to $s_i$ under $E$ is a subterm of $t'_j$, a contradiction.  Hence in fact no substitutions of the form $s_i/s'_i$ occur.  But then no $E'$ substitutions occur, since no $s_i$ is equivalent under $E$ to a subterm of $t_j$, so $t'_j\in \congclos_E(\{t_j\})$, which is a contradiction, so the claim is proved. \dm{This paragraph is probably not very easy to undersand}

To complete the proof of Lemma \ref{lem:ignoreinf} it remains to show that the $s_i$ can be chosen in the desired way.  

\begin{lemma}\label{lem:strongmin}
Let $E$ be a finite set of equalities and $s$ any term.  Then $\congclos_E(s)$ contains only finitely many strongly minimal elements.
\end{lemma}
\begin{proof}
Let $T$ be the set of terms appearing in $E$.  For $S\subseteq T$, write $[t]_S$ for the set of elements of $\congclos_E(t)$ in which elements of $\congclos(S)$ do not appear as subterms.  We will show by downwards induction that for all $t$ and all $S$, $[t]_S$ contains only finitely many strongly minimal elements.  The base case $S=T$ is trivial, since $[t]_T\subseteq \{t\}$.

Let $t'$ be a strongly minimal element of $[t]_S$.  Let $t_1,\ldots,t_k$ be maximal subterms of $t'$ equivalent to elements of $T$, so that $t'=C[t_1/X_1,\ldots,t_k/X_k]$ for some context $C$, and we have $\congclos_E(t') = C[\congclos_E(t_1)/X_1,\ldots,\congclos_E(t_k)/X_k]$, and hence in particular $[t]_S=[t']_S=C[[t_1]_S/X_1,\ldots,[t_k]_S/X_k]$.  Let $t''=C[t'_1/X_1,\ldots,t'_k/X_k]$ be a strongly minimal element of $[t]_S=[t']_S$, with $t'_i\in [t_i]_S$.  Then each $t'_i$ is strongly minimal, so $t_i$ cannot appear as a subterm of $t'_i$, so $t'_i\in [t_i]_{S\cup\{t_i\}}$.  Hence strongly minimal elements of $[t]_S$ are contained in $C[[t_1]_{S\cup\{t_1\}}/X_1,\ldots,[t_k]_{S\cup\{t_k\}}/X_k]]$.  By the inductive hypothesis each $[t_i]_{S\cup \{t_i\}}$ contains only finitely many strongly minimal elements and hence so does $[t]_S$.
\end{proof}

\begin{lemma}\label{lem:strongminsub}
Let $E$ be a finite set of equalities and $s,t$ any terms.  If $t$ is a subterm of an element of $\congclos_E(s)$ then $t$ is equivalent under $E$ to a subterm of \emph{either} a strongly minimal element of $\congclos_E(s)$ \emph{or} a term appearing in $E$.
\end{lemma}
\begin{proof}
Let $s'$ be an term in $\congclos_E(s)$ of minimum size among terms which contain a subterm equivalent to $t$; say that $t' \in \congclos_E(t)$ is a subterm of $s'$.  If $s'$ is strongly minimal then we are done.  Otherwise there is a subterm $s''$ of $s'$ and a sequence of $E$-substitutions which replaces $s''$ with some strict subterm $s'''$, so $s'=C[s''/X]$ is equivalent to $C[s'''/X]$.  If the occurrence of $t'$ is not contained in any of the substituted terms then some $t''$ equivalent to $t'$ is a subterm of $C[s'''/X]$, which contradicts minimality (since $C[s'''/X]$ is smaller than $C[s''/X]$).  On the other hand if it is then some $t''$ equivalent to $t'$ is a subterm of a term appearing in $E$, as required.
\end{proof}

Combining these lemmas gives the result that the downwards-closure of any equivalence class meets only finitely many equivalence classes.

\begin{corollary}\label{cor:downfin}
Let $E$ be a finite set of equalities and $s$ any term.  Then the downwards-closure of $\congclos_E(s)$ (i.e. the set of subterms of elements of $\congclos_E(s)$) contains only finitely many non-equivalent terms.
\end{corollary}
\begin{proof}
By Lemma \ref{lem:strongminsub} each equivalence class of the downwards-closure of $\congclos_E(s)$ is represented by a subterm of either a strongly minimal element of $\congclos_E(s)$ or a term appearing in $E$.  But $E$ is finite so only finitely many terms appear in $E$, and by Lemma \ref{lem:strongmin} $\congclos_E(s)$ contains only finitely many strongly minimal terms.  Each term has only finitely many subterms, so the downwards-closure of $\congclos_E(s)$ contains only finitely many equivalence classes.
\end{proof}

We can now conclude the proof of Lemma \ref{lem:ignoreinf} by using Corollary \ref{cor:downfin} to show that it is possible to choose the $s_i$ in the required way: that is, so that $\congclos_E(s_i)$ does not meet the downwards-closure of $S=\bigcup_j \congclos_E(t_j) \cup \congclos_E(t'_j) \cup \bigcup_{i'} \congclos_E(s'_{i'}$, or the downwards-closure of $\congclos_E(s_{i'})$ for any $i'\neq i$.

\begin{lemma}\label{lem:disjsat}
The problem of determining whether $\bigvee T$ is satisfiable, where 
\[T = \left\{s_1=t_1 \wedge \ldots \wedge s_n=t_n \wedge s'_1 \neq t'_1 \wedge \ldots \wedge s'_m \neq t'_m \mid s_i \in S_i, t_i \in S'_i, s'_j\in T_j, t'_j\in T'_j\right\},\]
where $S_1,S'_1,\ldots,S_n,S'_n,T_1,T'_1,\ldots,T_m,T'_m$ are given regular sets of terms, is decidable.
\end{lemma}
\end{comment}


